Sharp Constants in Uniformity Testing via the Huber Statistic

Uniformity testing is one of the most well-studied problems in property testing, with many known test statistics, including ones based on counting collisions, singletons, and the empirical TV distance. It is known that the optimal sample complexity to distinguish the uniform distribution on $m$ elements from any $\epsilon$-far distribution with $1-\delta$ probability is $n = \Theta\left(\frac{\sqrt{m \log (1/\delta)}}{\epsilon^2} + \frac{\log (1/\delta)}{\epsilon^2}\right)$, which is achieved by the empirical TV tester. Yet in simulation, these theoretical analyses are misleading: in many cases, they do not correctly rank order the performance of existing testers, even in an asymptotic regime of all parameters tending to $0$ or $\infty$. We explain this discrepancy by studying the \emph{constant factors} required by the algorithms. We show that the collisions tester achieves a sharp maximal constant in the number of standard deviations of separation between uniform and non-uniform inputs. We then introduce a new tester based on the Huber loss, and show that it not only matches this separation, but also has tails corresponding to a Gaussian with this separation. This leads to a sample complexity of $(1 + o(1))\frac{\sqrt{m \log (1/\delta)}}{\epsilon^2}$ in the regime where this term is dominant, unlike all other existing testers.

==> empty_bins_n_o_m.tex <==
\begin{assumption}
$n = o(m)$ and $m = o(n^2)$
\end{assumption}

Let our statistic $S_n^* = \sum_{j=1}^m I \{n \Gamma_j^n = 0\}$.

Note that by the lemma in paper, $$E[S_n^*]= m - n + \frac{1}{2} \frac{n^2}{m} (m \sum_{j=1}^m \nu_j^2) + O(\frac{n^3}{m^2})$$


We will analyze the statistic $$\Tilde{S}_n^* = 2m - 2\sum_{j=1}^m I\{n \Gamma_j^n = 0\} - 2n$$

which has expectation $$E[\Tilde{S}_n^*] = -\frac{n^2}{m} (m \sum_{j=1}^m \nu_j^2) + O(\frac{n^3}{m^2})$$

Let $\P_m^b = \{\max_j q_j \le \gamma/m\}$ for constant $\gamma$ satisfying $\gamma \ge \max\{2/(1-\eps), 4 \eps\}$.

\begin{proposition}
For any $\nu \in \P_m^b$, the log MGF for the statistic $\Tilde{S}_n^*$ has the following asymptotic expansion

$$\Lambda_{\nu, \Tilde{S}_n^*}(\theta) = \frac{1}{2} \frac{n^2}{m} (m \sum_{j=1}^m \nu_j^2)(e^{-2\theta} - 1) + O(\frac{n^3}{m^2}) + O(1)$$
\end{proposition}
The MGF is given by $$e^{2\theta m} e^{-2\theta n} \frac{n!}{2\pi i} \oint g(\lam) d\lam$$

where

$$g(\lam) = e^\lam \prod_{j=1}^m (1 - e^{-\lam \nu_j} + e^{-\lam \nu_j} e^{-2\theta}) \frac{1}{\lam^{n+1}} = \prod_{j=1}^m (e^{\lam \nu_j} - 1 + e^{-2\theta}) \frac{1}{\lam^{n+1}}$$

$$\frac{d}{d\lam}g(\lam) = g(\lam)[\sum_{j=1}^m \frac{\nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} - \frac{n+1}{\lam}]$$

Select point close to saddle point defined as solution to $$\sum_{j=1}^m \frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} = n$$

Observe that there is a unique real-valued non-negative solution $\lambda_0$ since the LHS is continuous and strictly increasing function of $\lam$ and is $0$ when $\lam = 0$ and goes to $\infty$ as $\lam$ goes to $\infty$.

Now, %note that since $e^{-\lam \nu_j} \ge 1 - \lam \nu_j$, we have that when $\theta \le 0$, $e^{-2\theta} \ge 1$, and so, 

$$\frac{e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} = \frac{1}{1 - e^{-\lam \nu_j} + e^{-\lam \nu_j} e^{-2\theta}} = \frac{e^{2\theta}}{e^{2\theta} - e^{-\lam \nu_j} e^{2\theta} + e^{-\lam \nu_j}}$$

Now, note that when $\theta \le 0$, $e^{-2\theta} \ge 1$, and $e^{2\theta} \le 1$. Thus, the above is at least $$ \frac{e^{2\theta}}{1 - e^{-\lam \nu_j}[1 - e^{2\theta}]}$$ 

Using Taylor series of $1/(1-x)$, we have that the above is at least $$e^{2\theta} (1 + e^{-\lam \nu_j} [1 - e^{2\theta}]) \ge e^{2\theta}$$ since the second term is positive. Similarly, when $\theta \ge 0$, this expression is at most $e^{2\theta}$.

Now, when $\theta \le 0$, note that $e^{-2\theta} \ge 1$, and so, $$\frac{e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} \le \frac{e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + 1} = 1$$

Similarly when $\theta \ge 0$, this expression is at least $1$.

Thus, finally, we have the following. When $\theta \le 0$,

$$ e^{2\theta} \le \frac{e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} \le 1$$

And so, $$n e^{2\theta} \le \lam_0 \le n$$

And when $\theta \ge 0$, we have that $$1 \le \frac{e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} \le e^{2\theta}$$

And so, $$n \le \lam_0 \le ne^{2\theta}$$

Thus, $\lam_0 = O(n)$. So, since $\nu \in \mathcal{P}_m^b$, we have that $\lam_0 \nu_j = o(1)$. Thus, we have that the denominator satisfies $$e^{\lam_0 \nu_j} - 1 + e^{-2\theta} = e^{-2\theta} + o(1)$$. Substituting into the saddle point equation, we get that $$\sum_{j=1}^m \lam_0 \nu_j e^{\lam_0 \nu_j} = n(e^{-2\theta} + o(1))$$

This means that $\lam_0 = ne^{-2\theta}(1 + o(1))$.

Let $w = \lam_0 e^{2\theta}/n - 1$ so that $\lam_0 = ne^{-2\theta}(1+w)$. We will find a refined approximation for $w$. Since $\lam_0 \nu_j = O(\frac{n}{m})$, we have that numerator and denominator satisfy

$$\lam_0 \nu_j e^{\lam_0 \nu_j} = \lam_0 \nu_j (1 + \lam_0 \nu_j + O(\frac{n^2}{m^2}))$$

$$e^{\lam_0 \nu_j} - 1 + e^{-2\theta} = e^{-2\theta} + \lam_0 \nu_j + O(\frac{n^2}{m^2})$$

Thus, we have that $$\sum_{j=1}^m \frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{-2\theta}} = \sum_{j=1}^m \frac{e^{2\theta} \lam_0 \nu_j (1 + \lam_0 \nu_j + O(\frac{n^2}{m^2}))}{1 + e^{2\theta} \lam_0 \nu_j + O(\frac{n^2}{m^2})}$$

$$= \sum_{j=1}^m e^{2\theta} \lam_0 \nu_j (1 + \lam_0 \nu_j + O(\frac{n^2}{m^2}))(1 - e^{2\theta} \lam_0 \nu_j + O(\frac{n^2}{m^2})) = \sum_{j=1}^m [e^{2\theta} \lam_0 \nu_j + \lam_0^2\nu_j^2(e^{2\theta} - e^{4\theta}) + O(\frac{n^3}{m^3})]$$

So, we have that $$w + n \sum_{j=1}^m \nu_j^2 (1+w)^2 (e^{-2\theta} - 1) = O(\frac{n^2}{m^2})$$

So, $$w = n\sum_{j=1}^m \nu_j^2 (1-e^{-2\theta})(1 + O(\frac{n}{m})) = O(\frac{n}{m})$$

Thus, $\lam_0 = ne^\theta (1 + O(\frac{n}{m}))$

Now, the integral we want to evaluate is $$e^{2\theta m} e^{-2\theta n} \frac{n!}{2 \pi i} \lam_0^{-n} \int_{-\pi}^\pi h(\psi) d\psi$$

Where $$h(\psi) = e^{-n i \psi} \prod_{j=1}^m (e^{\lam_0 \nu_j e^{i \psi}} - 1 + e^{-2\theta})$$

Now, we will approximate $h(\psi)$

$$h(\psi) = e^{-n i \psi} \prod_{j=1}^m (-1 + e^{-2\theta} + 1 + \lam_0 \nu_j e^{i \psi} + O(\frac{n^2}{m^2})) = e^{-ni\psi} \prod_{j=1}^m (e^{-2\theta} + \lam_0 \nu_j e^{i \psi} + O(\frac{n^2}{m^2}))$$

$$ = e^{-i n \psi} \exp\{\sum_{i=1}^m [\log(e^{-2\theta}) +  \log(1 + \lam_0 \nu_j e^{i \psi} e^{2\theta} + O(\frac{n^2}{m^2}))]\}$$

$$= e^{-i n \psi} \exp\{\sum_{i=1}^m (-2\theta + \lam_0 \nu_j e^{i\psi} e^{2\theta} + O(\frac{n^2}{m^2}))\}$$

$$ = e^{-i n \psi} \exp\{-2m \theta + \lam_0 e^{i \psi} e^{2\theta} + O(\frac{n^2}{m})\}$$

$$= e^{-i n \psi} e^n \exp\{-2m \theta - n (1 - e^{i \psi}) + O(\frac{n^2}{m})\}$$

Let $H(\psi) = \log(h(\psi))$. Thus, $$H(\psi) = -in \psi + \sum_{j=1}^m \log(e^{-2\theta} - 1 + \exp\{\lam_0 \nu_j e^{i \psi}\})$$

$$H'(\psi) = -in + i \sum_{j=1}^m \frac{\lam_0 \nu_j e^{i \psi} \exp(\lam_0 \nu_j e^{i \psi})}{e^{-2\theta} - 1 + \exp\{\lam_0 \nu_j e^{i \psi}\}}$$

$$H''(\psi) = -\sum_{j=1}^m \exp\{\lam_0 \nu_j e^{i \psi}\} \times \frac{\lam_0 \nu_j e^{i \psi} (e^{-2\theta} - 1)(1 + \lam_0 \nu_j e^{i \psi}) + \lam_0 \nu_j e^{i \psi}\exp\{\lam_0 \nu_j e^{i \psi}\}}{(e^{-2\theta} - 1 + \exp\{\lam_0 \nu_j e^{i \psi}\})^2}$$

It's clear that $Im(H(0)) = 0$. It is also clear that $H'(0) = 0$. From $\lam_0 = n e^\theta(1+w)$, it follows that $$Re(H(0)) = \sum_{i=1}^m [-2\theta + \log(1 + \lam_0 \nu_j e^{2\theta} + \frac{1}{2} \lam_0^2 \nu_j^2 e^{2\theta})]$$

$$=  -2m \theta + n(1+w) - \frac{(1- e^{-2\theta})n^2 (\sum_j \nu_j^2)}{2} + O(\frac{n^3}{m^2})$$

$$H''(\psi) = -ne^{i \psi} + O(\frac{n^2}{m})$$

Note that for large enough $n$ and $\psi \in [-\pi/3, \pi/3]$, we have $Re(H''(\psi)) \le -0.4n$. Then, by mean value theorem,

$$Re(H(\psi)) \le H(0) - 0.2 n \psi$$

Then, for large enough $n, m$,

$$I_1 \le e^{H(0)} \int_{-\pi/3}^{\pi/3} e^{-0.2 n \psi^2} d\psi \le e^{H(0)} \int_{-\infty}^{\infty} e^{-0.2 n \psi^2} d \psi = e^{H(0)} \frac{\sqrt{\pi}}{\sqrt{0.2 n}}$$

To lower bound $I_1$, note that $Im(H''(\psi)) = -n \sin(\psi) + O(\frac{n^2}{m})$, so that since $|\sin(\psi)| \le |\psi|$, we have that for large $n$ and any $\psi \in [-\pi/3, \pi/3]$, $|Im(H''(\psi))| \le 1.1 n |\psi|$. Also, clearly $Re(H''(\psi)) \ge -1.1n$. So, applying mean value theorem, there exists some $c > 0$ such that for $\psi \in [-\pi/3, \pi/3]$, $$Re(H(\psi)) \ge H(0) - 1.1n \psi^2$$

 Lower bound is same as in paper. Thus, $$I_1 = e^{H(0)}\frac{1}{\sqrt{n}} e^{O(1)} = e^{-2m\theta} e^{n(1+o(1))} \frac{1}{\sqrt{n}} e^{O(1)}$$
 
 Also, as in the paper, $I_2$ and $I_3$ are much smaller than $I_1$. So, $$E_\nu[\exp\{\theta(\tilde{S}_n^*)\}]  = \frac{n!}{2\pi} \lam_0^{-n} e^{2 \theta m} e^{-2 \theta n} I_1 (1+o(1))$$
 
 $$ = \frac{n!}{2 \pi} \lam_0^{-n} e^{2\theta m} e^{-2\theta n} e^{H(0)} \frac{1}{\sqrt{n}} e^{O(1)} (1+o(1))$$

$$ = \frac{e^n n!}{n^n \sqrt{2 \pi n}} (1 + n \sum_j \nu_j^2 (1 - e^{-2\theta}) + O(\frac{n^2}{m^2}))^{-n} \times \exp\{-\frac{1}{2} n^2 (\sum_{j=1}^m \nu_j^2) (1 - e^{-2\theta}) + O(\frac{n^3}{m^2})\} e^{O(1)}$$

$$ = \frac{n!e^n}{n^n \sqrt{2 \pi n}} \exp\{-\frac{1}{2} n^2 (\sum_{j=1}^m \nu_j^2)(1 - e^{-2\theta}) + O(\frac{n^3}{m^2})\} e^{O(1)}$$

 Finally, since by Stirling's formula, $\frac{n! e^n}{n^n \sqrt{2\pi n}} = 1 + O(\frac{1}{n})$, log MGF is $$\frac{1}{2} \frac{n^2}{m} (m \sum_{j=1}^m \nu_j^2)(e^{-2\theta} - 1) + O(\frac{n^3}{m^2}) + O(1)$$

\subsection{Log MGF for distributions not in $\mathcal{P}_m^b$}
Fix small constant $\eta > 0$ and consider set of indices $S_0 := \{j \in [m] : q_j \ge \gamma/m\}$. Since $q \not\in \mathcal{P}_m^b$, $S_0$ is non-empty. Denote $$W_\eta(q) = \{j : n q_j \ge \eta\}, \beta(q) = \sum_{j \in W_\eta(q)}q_j$$

Now, for $j \not \in W_\eta$, $$\frac{\lam_0 \nu_j e^{\lam_0 \nu_j}}{e^{\lam_0 \nu_j} - 1 + e^{-2\theta}} = e^{2\theta} \lam_0 \nu_j + \lam_0^2 \nu_j^2(e^{2\theta} - e^{4\theta})(1 + o^\eta(1))$$

For $j \in W_\eta$, we have $$\frac{\lam_0 \nu_j e^{\lam_0 \nu_j}}{e^{\lam_0 \nu_j} - 1 + e^{-2\theta}} = D_j \lam_0 \nu_j e^{2\theta}$$
where $$D_j := \frac{e^{-2\theta}}{1 - e^{-\lam_0\nu_j} + e^{-2\theta} e^{-\lam_0 \nu_j}} \ge e^{-2\theta}$$

Thus, $$\sum_{j=1}^m \frac{\lam_0 \nu_j e^{\lam_0 \nu_j}}{e^{\lam_0 \nu_j} - 1 + e^{-2\theta}} = \lam_0 (1 + \sum_{j \in W_\eta} \nu_j (D_j - 1)) e^{2\theta} + \lam_0^2 \sum_{j \not \in W_\eta} \nu_j^2 (e^{2\theta} - e^{4\theta})(1 + o^\eta(1)) = n$$

Thus, $$\lam_0 = \frac{n e^{-2\theta}}{1 + \sum_{j \in W_\eta} \nu_j(D_j - 1)} (1 +w)$$

where $w = o^\eta(1)$.

\textbf{Lemma }
For sufficiently small $\eta >0$, any $\theta \in [-1, 0)$ and $\beta > 0$ there exists $n_0$ such that for any $n > n_0$, and any $\nu$ such that $\beta(\nu) > \beta$, $$\Gamma_{nu, \tilde{S_n}^*}(\theta) \le -\beta(\nu) \alpha(\theta) n$$

\textbf{Proof of Prop 6}

We will bound $Re(H(\psi))$ by $H(0) = \sum_{j=1}^m \log(e^{-2\theta} - 1 + \exp\{\lam_0 \nu_j e^{i \psi}\})$. For $\psi \in [-\pi/2, \pi/2]$

$$Re[\log(e^{-2\theta} - 1 + e^{\lam_0 \nu_j e^{i \psi}})] = Re[\log(e^{\lam_0 \nu_j e^{i\psi}}) + \log(e^{-\lam_0 \nu_j e^{i \psi}}(e^{-2\theta} - 1) + 1)]$$

$$\le \lam_0 \nu_j \cos \psi + \log(e^{-\lam_0 \nu_j \cos\psi} (e^{-2\theta} - 1) + 1)$$

So, by the same inequality as in paper, $$Re(H(\psi)) \le H(0)$$

For other values of $\psi$, $|e^{\lam_0 \nu_j e^{i \psi}}| \le 1$. Thus, $$Re[\log(e^{-2\theta} - 1 + e^{\lam_0 \nu_j e^{i \psi}})] \le \log(e^{-2\theta}) = -2\theta$$

But this is less than the above expression at $cos\psi = 0$, which in turn is less than $H(0)$. Thus, finally for all values of $\psi$, $$Re(H(\psi)) \le H(0)$$

We now approximate $H(0)$. For $j \not \in W_\eta$, $$\log(e^{-2\theta} - 1 + \exp(\lam_0 \nu_j)) = -2\theta +  \lam_0 \nu_j e^{2\theta} + \frac{1}{2} \lam_0^2 \nu_j^2 (e^{2\theta} - e^{4\theta})(1+o^\eta(1))$$

%For $j \in W_\eta$, we have $$\log(e^{-2\theta} - 1 + \exp(\lam_0 \nu_j)) = -2\theta + 2e^{2\theta} + 

Now, $$E_\nu[\exp\{\theta(\tilde{S}_n^*)\}] \le \frac{n!}{2\pi} \lam_0^{-n}e^{2\theta m} e^{-2\theta n} \exp\{H(0)\}$$

$$\le n! \lam_0^{-n} e^{2\theta m} e^{-2\theta n} \exp\{\sum_{j \not\in W_\eta}[-2\theta + \lam_0 \nu_j e^{2\theta} + \frac{1}{2} \lam_0^2 \nu_j^2(e^{2\theta} -e^{4\theta})(1+o^\eta(1))]\}$$

$$\times \exp\{\sum_{j \in W_\eta}[-2\theta + \lam_0 \nu_j e^{2\theta} + e^{2\theta}(\exp\{\lam_0 \nu_j\} - \lam_0 \nu_j - 1)]\}$$

$$ = \frac{n! e^n}{n^n} (1 + \sum_{j \in W_\eta} (D_j - 1))^n (1+w)^{-n}\exp\{-\frac{\frac{1}{2} n^2 \sum_{j \not\in W_\eta} \nu_j^2 (1 - e^{-2\theta})(1 + o^\eta(1))}{1 + \sum_{j \in W_\eta} \nu_j(D_j - 1)}\}$$

$$\times \exp\{n[\frac{(1+w) + \sum_{j \in W_\eta} \nu_j (\exp\{\lam_0 \nu_j\} - \lam_0 \nu_j - 1)}{1 + \sum_{j \in W_\eta} \nu_j (D_j - 1)}]\}$$

So finally we need to bound $$\sum_{j \in W_\eta} \nu_j(D_j - 1) - 1 + \frac{1 + \sum_{j \in W_\eta} \nu_j(\exp(\lam_0 \nu_j) - \lam_0 \nu_j - 1)}{1 + \sum_{j \in W_\eta} \nu_j(D_j - 1)}$$

$$ = \frac{(\sum_{j \in W_\eta} (D_j - 1))^2 + \sum_{j \in W_\eta} \nu_j(\exp(\lam_0 \nu_j) - \lam_0 \nu_j - 1)}{1 + \sum_{j \in W_{\eta}} \nu_j (D_j - 1)}$$

\section{Trying when $n = o(\frac{m}{\eps^4})$}

Conditions:

$$n = o(\frac{m}{\eps^4})$$

$$\frac{\sqrt{m}}{\eps^2} = o(n)$$

$$m = o(\frac{1}{\eps^4})$$


$$g(\lam) = e^\lam \prod_{j=1}^m [e^{\frac{\theta}{m}} e^{-\lam \nu_j} \sum_{k \le \floor{\frac{n}{m}}} \frac{(\lam \nu_j e^{\frac{\theta}{n}})^k}{k!} + e^{-\frac{\theta}{m}} e^{-\lam\nu_j} \sum_{k > \floor{\frac{n}{m}}} \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!}]\frac{1}{\lam^{n+1}}$$

$$ = e^\lam \prod_{j=1}^m [e^{-\lam \nu_j} \sum_{k \le \floor{\frac{n}{m}}}[ e^{\frac{\theta}{m}} \frac{(\lam \nu_j e^{\frac{\theta}{n}})^k}{k!} - e^{-\frac{\theta}{m}} \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!} ] + e^{-\lam\nu_j} e^{-\frac{\theta}{m}} e^{\lam \nu_j e^{\frac{-\theta}{n}}}]\frac{1}{\lam^{n+1}}$$

$$ = \prod_{j=1}^m [\sum_{k \le \floor{\frac{n}{m}}} [e^{\frac{\theta}{m}} \frac{(\lam \nu_j e^{\frac{\theta}{n}})^k}{k!} - e^{-\frac{\theta}{m}} \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!} ] + e^{-\frac{\theta}{m}} e^{\lam \nu_j e^{\frac{-\theta}{n}}}]\frac{1}{\lam^{n+1}}$$

Now $$\frac{d}{d\lam} g(\lam) = g(\lam) \{\sum_{j=1}^m [\frac{\sum_{k \le \floor{\frac{n}{m}}} [e^{\frac{\theta}{m}} \frac{k}{\lam} \frac{(\lam\nu_j e^{\frac{\theta}{n}})^k}{k!} - e^{-\frac{\theta}{m}} \frac{k}{\lam} \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!}] + \nu_j e^{-\frac{\theta}{m}} e^{\lam \nu_je^{-\frac{\theta}{n}}}}{\sum_{k \le \floor{\frac{n}{m}}}[e^{\frac{\theta}{m}} \frac{(\lam \nu_j e^{\frac{\theta}{n}})^k}{k!} - e^{-\frac{\theta}{m}} \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!} ] + e^{-\frac{\theta}{m}} e^{\lam \nu_j e^{\frac{-\theta}{n}}}}] - \frac{n+1}{\lam}\}$$

So, setting to $0$, we want solution to $$\sum_{j=1}^m [\frac{\sum_{k \le \floor{\frac{n}{m}}} [e^{\frac{\theta}{m}} k \frac{(\lam\nu_j e^{\frac{\theta}{n}})^k}{k!} - e^{-\frac{\theta}{m}} k \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!}] + \lam \nu_j e^{-\frac{\theta}{m}} e^{\lam \nu_je^{-\frac{\theta}{n}}}}{\sum_{k \le \floor{\frac{n}{m}}}[e^{\frac{\theta}{m}} \frac{(\lam \nu_j e^{\frac{\theta}{n}})^k}{k!} - e^{-\frac{\theta}{m}} \frac{(\lam \nu_j e^{-\frac{\theta}{n}})^k}{k!} ] + e^{-\frac{\theta}{m}} e^{\lam \nu_j e^{\frac{-\theta}{n}}}}] = n$$

\section{Trying when $n = \Theta(m)$}

Three conditions: $$n = o(\frac{m}{\eps^2})$$

$$m = o(n^2 \eps^4)$$

$$\eps = o(1)$$

Optimal $\theta = O(\eps^2)$

Consider the statistic $$S_n^* = \sum_{j=1}^m I\{n \Gamma_j^n = 0\}$$

We have that $$E[S_n^*] = \sum_{j=1}^m (1 - \nu_j)^n$$

Note that for the uniform distribution $$E[S_n^*] = m (1- \frac{1}{m})^n = m (e^{-1/m} - \frac{1}{2m^2} + O(\frac{1}{m^3}))^n = m (e^{-n/m} - \frac{n}{2m^2} e^{-n/m} + O(\frac{1}{m^2}))$$

$$ = m e^{-n/m} - \frac{n}{2m} e^{-n/m} + O(\frac{1}{m})$$

So, consider the statistic $\Tilde{S}_n^* = S_n^* - m e^{-n/m} - \frac{n}{2m} e^{-n/m}$. It has expectation $O(1/m)$.


First consider $\nu \in \P_m^b$ where $\P_m^b = \{q \in \P_m : \max_j q_j \le \gamma/m\}$ for constant $\gamma$.

The MGF of $\Tilde{S}_n^*$ is given by 

$$E_\nu [\exp\{ \theta (\Tilde{S}_n^*)\}] = e^{-m e^{-n/m} \theta} e^{-\frac{n}{2m}e^{-n/m} \theta} \frac{n!}{2 \pi i} \oint g(\lam) d \lam$$

where $$g(\lam) = e^\lam \prod_{j=1}^m (1 - e^{-\lam \nu_j} + e^{-\lam \nu_j} e^{\theta}) \frac{1}{\lam^{n+1}} = \prod_{j=1}^m [e^{\lam \nu_j} - 1 + e^\theta] \frac{1}{\lam^{n+1}}$$

As in the previous case, 

$$g(\lambda) = g(\lambda)[\sum_{j=1}^m \frac{\nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} -1 + e^{\theta}} - \frac{n+1}{\lam}]$$

So, again, we want the solution to $$\sum_{j=1}^m \frac{\lam \nu_je^{\lam \nu_j}}{e^{\lam\nu_j} - 1 + e^{\theta}} = n$$

Following same argument, we have that $\lam_0 = O(n)$.

Now, note that the denominator $$e^{\lam \nu_j} -  1 + e^{\theta} = e^{\lam \nu_j} + O(\theta)$$

Now, this means that since $\lam_0 = O(n)$, which means that $\lam_0 \nu_j = O(1)$, $$\sum_{j=1}^m \frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{\theta}} = \sum_{j=1}^m \frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} + O(\theta)} = \sum_{j=1}^m \frac{\lam \nu_j}{1 + O(\theta) e^{O(1)}} = \sum_{j=1}^m \frac{\lam\nu_j}{1 + O(\theta)}$$

Thus, $$\lam_0 = n(1 + O(\theta))$$

Let $w = \lam_0/n - 1$ so that $\lam_0 = n(1 + w)$

We know that $w = O(\theta)$. We will obtain a more precise approximation. Note that $$\frac{\lam\nu_j e^{\lam \nu_j}}{e^{\lam\nu_j} - 1 + e^{\theta}} = \frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} + \theta + O(\theta^2)} = \frac{\lam \nu_j}{1 + e^{-\lam \nu_j} \theta + O(\theta^2)} = \lam \nu_j - \theta e^{-\lam \nu_j} \lam \nu_j + O(\theta^2)$$

Now $$\sum_{j=1}^m [\lam \nu_j  - \theta e^{-\lam \nu_j} \lam \nu_j + O(\theta^2)] = n$$

Now, substituting $\lam_0 = n(1+w)$, we get $$n(1+w) - \theta n (1+w) \sum_{j=1}^m e^{-\lam \nu_j} \nu_j + m * O(\theta^2) = n$$

Thus, $$w - \theta (1+w) \sum_{j=1}^m e^{-\lam \nu_j} \nu_j + \frac{m}{n} * O(\theta^2) = 0$$

Since $\frac{m}{n} = O(1)$, this gives us that $$w[1 - \theta \sum_{j=1}^m e^{-\lam \nu_j} \nu_j] = O(\theta^2) + \theta \sum_{j=1}^m e^{-\lam \nu_j} \nu_j$$

Note that if $n = o(m)$ the above no longer holds. It still holds if $m = o(n)$.

Note that $$\sum_{j=1}^m e^{-\lam \nu_j} \nu_j = O(1)$$

Thus, we have $$w (1 + O(\theta)) = \theta \sum_{j=1}^m e^{-\lam \nu_j} \nu_j + O(\theta^2)$$
$$w = \theta \sum_{j=1}^m e^{-\lam \nu_j} \nu_j + O(\theta^2) = \theta \sum_{j=1}^m e^{-n \nu_j} \nu_j + O(\theta^2)$$

%Let $w_1 = \theta \sum_{j=1}^m e^{-n \nu_j} \nu_j$
%
%%Now, since $\nu_j = \frac{c + d\eps}{m}$, ${\color{red} \text{assumption on } \nu_j \text{ used here }}$we have that $$w_1 = -2\theta \sum_{j=1}^m e^{-\frac{cn}{m}} e^{O(\eps)} \nu_j + O(\eps^2) = - 2\theta e^{-\frac{cn}{m}} + O(\eps^2)$$
%
%Let $w_2$ be so that $\lam_0 = n(1 + w_1 + w_2)$ where $w_2$ will be the $O(\theta^2)$ term.
%
%Note that $$\frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} - 1 + e^{\theta}} = \frac{\lam \nu_j e^{\lam \nu_j}}{e^{\lam \nu_j} +\theta + \theta^2/2 + O(\theta^3)} = \frac{\lam \nu_j}{1 + \theta e^{-\lam \nu_j} + \frac{1}{2} \theta^2 e^{-\lam \nu_j} + O(\theta^3)}$$
%
%$$ = \lam \nu_j[1 - \theta e^{-\lam \nu_j} - \frac{1}{2} \theta^2 e^{-\lam \nu_j} + \theta^2 e^{-2 \lam \nu_j} + O(\theta^3)]$$
%
%So, $$\sum_{j=1}^m [\lam \nu_j - \theta \lam \nu_j e^{-\lam \nu_j} + \lam \nu_j \theta^2 [-\frac{1}{2} e^{-\lam \nu_j} + e^{-2\lam \nu_j}] + O(\theta^3)] = n$$
%
%So, $$(w_1 + w_2) - \theta (1 + w_1 + w_2) \sum_{j=1}^m \nu_j e^{-\lam \nu_j} + \theta^2 (1 + w_1 + w_2) \sum_{j=1}^m[\nu_j e^{-2 \lam \nu_j} - \frac{1}{2} \nu_j e^{-\lam \nu_j}] = 0$$
%
%Since $w_1 = \theta \sum_{j=1}^m e^{-\lam \nu_j} \nu_j$, we get $$w_2 - \theta (w_1 + w_2) \sum_{j=1}^m \nu_j e^{-\lam \nu_j} + \theta^2(1 + w_1 + w_2) \sum_{j=1}^m [\nu_j e^{-2 \lam \nu_j} - \frac{1}{2} \nu_j e^{-\lam \nu_j}] = 0$$
%
%Thus, $$w_2 - \theta^2 [\sum_{j=1}^m \nu_j e^{-\lam \nu_j}]^2 + \theta^2 \sum_{j=1}^m [\nu_j e^{-2 \lam \nu_j} - \frac{1}{2} \nu_j e^{-\lam \nu_j}] + O(\theta^3) = 0$$
%
$$w_2 = \theta^2 [(\sum_{j=1}^m \nu_j e^{-\lam \nu_j})^2 + \sum_{j=1}^m [- \nu_j e^{-2\lam \nu_j} + \frac{1}{2} \nu_j e^{-\lam \nu_j}]] + O(\theta^3)$$

Now, we will evaluate the integral along the closed contour given by $\lam = \lam_0 e^{i \psi} = n(1 + w) e^{i\psi}$

$$E_\nu[\exp(\theta (\Tilde{S}_n^*))] = e^{-m e^{-n/m} \theta} e^{-\frac{n}{2m} e^{-n/m} \theta} \frac{n!}{2\pi} \int_{-\pi}^\pi g(\lam_0 e^{i \psi}) \lam_0 e^{i \psi} d \psi$$

$$ = \frac{n!}{2\pi} \lam_0^{-n} e^{-m e^{-n/m} \theta} e^{-\frac{n}{2m}e^{-n/m} \theta} Re[\int_{-\pi}^\pi h(\psi) d\psi ]$$

where $$h(\psi) = e^{-i n \psi} \prod_{j=1}^m ((e^\theta - 1) e^{i \psi} + e^{\lam_0 \nu_j e^{i \psi}})$$

Let $H(\psi) = \log(h(\psi))$. Then, $$H(0) = \sum_{j=1}^m \log( (e^{\theta} - 1)  + \exp(\lam_0 \nu_j ))$$
%Note that $$e^{-\lam \nu_j} = e^{-\frac{cn}{m}} e^{-\frac{n}{m} [d\eps + w_1 c]} e^{O(\eps^2)} = e^{-\frac{cn}{m}} [1 - \frac{n}{m} [d \eps + w_1 c]] + O(\eps^2)$$ 

So, $$H(0) = \sum_{j=1}^m \log((\theta + \frac{\theta^2}{2} + O(\theta^3)) + \exp(\lam_0 \nu_j)) = \sum_{j=1}^m [\lam_0 \nu_j + \log(1 + e^{-\lam_0 \nu_j} (\theta + \frac{\theta^2}{2} + O(\theta^3)))]$$

$$ = \lam_0 + \sum_{j=1}^m[e^{-\lam_0 \nu_j} [\theta + \frac{\theta^2}{2}] - \frac{1}{2} e^{-2 \lam_0 \nu_j} \theta^2 + O(\theta^3)]$$

$$ = \lam_0 + \sum_{j=1}^m [n(\theta + (\theta w + \frac{\theta^2}{2})) \nu_j e^{-\lam_0 \nu_j} - \frac{1}{2} n^2 \nu_j^2 e^{-2 \lam_0 \nu_j} \theta^2 + O(\theta^3)]$$

$$ = \lam_0 + \sum_{j=1}^m [n \theta \nu_j e^{-\lam_0 \nu_j} + \{\theta^2 [\sum_{k=1}^m \nu_k e^{-n \nu_k}] + \frac{\theta^2}{2}\}\nu_j e^{-\lam_0 \nu_j} - \frac{1}{2}n^2 \nu_j^2 e^{-2\lam_0 \nu_j} \theta^2] + O(m \theta^3)$$

Note that $$e^{-\lam_0 \nu_j} = e^{-n(1 + w) \nu_j} = 1 - n(1 + w) \nu_j + \dots$$

$$ = [1 - n \nu_j + \frac{1}{2} n^2 \nu_j^2 - \dots] -n \nu_j w[1 - n \nu_j + \frac{n^2 \nu_j^2}{2} - \dots] $$

$$ = e^{-n \nu_j} - n \nu_j w e^{-n \nu_j} $$

$$ = e^{-n \nu_j} - n \nu_j e^{-n \nu_j}\theta [\sum_{k = 1}^m \nu_k e^{-n \nu_k}] $$

Similarly, $e^{-2 \lam_0 \nu_j} = e^{-2 n \nu_j} + O(\theta)$

Thus, $$H(0) = \lam_0 + \sum_{j=1}^m [n \nu_j (\theta e^{-n \nu_j} + (\theta^2 [\sum_{k=1}^m \nu_k e^{-n \nu_k}] (1 - n \nu_j e^{-n \nu_j})+ \frac{\theta^2}{2})) - \frac{\theta^2}{2} n^2 \nu_j^2 e^{-2 n \nu_j} + O(\theta^3)]$$

$$ = \lam_0 + \frac{n \theta^2}{2} + n \theta^2 [\sum_{k=1}^m \nu_k e^{-n \nu_k}] + \sum_{j=1}^m [n \nu_j \theta e^{-n \nu_j} - n^2 \nu_j^2 \theta^2 [\sum_{k=1}^m \nu_k e^{- n \nu_k}] e^{-n \nu_j} - \frac{\theta^2}{2} n^2 \nu_j^2 e^{-2n \nu_j}] + O(m \theta^3)$$


So now, we can evaluate the integral as $$E[\exp(\theta(\Tilde{S}_n^*))] = \frac{n!}{2\pi} \lam_0^{-n} e^{-m e^{-n/m} \theta} e^{-\frac{n}{2m} e^{-n/m} \theta} \frac{1}{\sqrt{n}} e^{H(0)} e^{O(1)} (1 + o(1))$$

$$ = $$

Finally, for the uniform distribution, $$\Lambda_{P_u, \Tilde{S}_n^*} =  \frac{n \theta^2}{2} + n\theta^2 e^{-n/m} - \frac{3\theta^2}{2} \frac{n^2}{m} e^{-2n/m} + O(m \theta^3)$$

So, $$\lim_{n \to \infty}\frac{m}{n^2 \eps^4} \Lambda_{u, \Tilde{S}_n^*} = t e^{-c}[\frac{1}{c} - \frac{1}{c^2}] +     t^2[\frac{1}{2c} + \frac{e^{-c}}{c} - \frac{3}{2} e^{-2c}]$$

Thus, $$\lim_{n \to \infty} \frac{m}{n^2 \eps^4} \log(Pr_u[S_n^* \ge E_u[S_n^*] + \frac{n^2\eps^2}{m} \tau]) = \lim_{n \to \infty} \frac{m}{n^2 \eps^4} \log(Pr_u[\Tilde{S}_n^* \ge E_u[S_n^*] - n e^{-n/m} + \frac{n^2 \eps^2}{m} \tau ])$$

$$ = \lim_{n \to \infty} \frac{m}{n^2 \eps^4} \log(Pr_u[\Tilde{S}_n^* \ge (m - n)e^{-n/m} + O(1) + \frac{n^2\eps^2}{m} \tau])$$

For the worst case distribution $$\Lambda_{q, \Tilde{S}_n^*} =  \frac{n \theta^2}{2} + n \theta^2 e^{-n/m} - \frac{3 \theta^2}{2} \frac{n^2}{m} e^{-2n/m} - 2 e^{-n/m} (2 m - n) \frac{n^2}{m^2} \theta \eps^2$$

So, $$\lim_{n \to \infty} \frac{m}{n^2 \eps^4} \Lambda_{q, \Tilde{S}_n^*} = t^2[\frac{1}{2c} + \frac{e^{-c}}{c} - \frac{3}{2} e^{-2c}] - 2e^{-c} [2 - c] t$$

We have $$\sum_{j=1}^m [\lam \nu_j + 2\theta e^{-\lam \nu_j} \lam \nu_j - 2 \theta^2 [e^{-2\lam\nu_j} (-2 + e^{\lam \nu_j}) \lam \nu_j] + O(\eps^3) ] = n$$

$$\lam + \sum_{j=1}^m [2 \theta e^{-\lam\nu_j} \lam \nu_j - 2 \theta^2 [e^{-\lam \nu_j} (-2 + e^{\lam \nu_j}) \lam \nu_j ] + O(\eps^3)] = n$$
$$w_1 + w_2 + \sum_{j=1}^m [2 \theta e^{-\lam\nu_j} \nu_j (1 + w_1 + w_2) - 2 \theta^2 [e^{-\lam \nu_j} (-2 + e^{\lam \nu_j}) \nu_j(1 + w_1 + w_2) ] ] = O(\eps^3)$$

Note that 
$$\sum_{j=1}^m [2\theta e^{-\lam \nu_j} \nu_j (1 + w_1 + w_2)] = e^{-\frac{cn}{m}}\sum_{j=1}^m [2\theta ( 1 - \frac{n}{m} (d \eps + w_1c) + O(\eps^2)) \nu_j (1 + w_1 + w_2)]$$

$$ = e^{-\frac{cn}{m}} [2 \theta (1 + w_1 + w_2) - 2\theta \frac{n}{m}(d\eps + w_1 c) (1 + w_1 + w_2) + O(\eps^3)]$$

$$ = e^{-\frac{cn}{m}} [2\theta + 2\theta [w_1 - \frac{n}{m} (d\eps + w_1 c)]] + O(\eps^3)$$

Also, $$\sum_{j=1}^m [2\theta^2 (e^{-\lam \nu_j} (-2 + e^{\lam \nu_j}) \nu_j (1 + w_1 + w_2))] = \sum_{j=1}^m [2\theta^2 (e^{-c\frac{n}{m}} + O(\eps)) (-2 + e^{\frac{cn}{m}} + O(\eps))\nu_j(1 + w_1 + w_2)]$$

$$ = 2\theta^2 [-2 e^{\frac{-cn}{m}} + 1] + O(\eps^3)$$

So, finally, $$w_1 + w_2 + 2\theta e^{-\frac{cn}{m}} [1 + w_1 - \frac{n}{m} (d\eps + w_1 c)] + 2\theta^2[-2 e^{-\frac{cn}{m}} + 1] = O(\eps^3)$$

So that $$w_2 = -w_1 - 2 \theta e^{-\frac{cn}{m}}[1 + w_1 - \frac{n}{m} (d \eps + w_1 c)] - 2 \theta^2 [-2 e^{\frac{-cn}{m}} + 1] + O(\eps^3)$$

$$ = -2 \theta e^{\frac{-cn}{m}}[w_1 - \frac{n}{m} (d \eps + w_1 c)] - 2 \theta^2 [-2 e^{\frac{-cn}{m}} + 1] + O(\eps^3)$$

Using Mathematica, $$\lam_0 = n(1 + 2 \theta e^{-\frac{n}{m}} + 2 \frac{\theta^2}{m} e^{-\frac{2n}{m}} (e^{n/m} m - 2n) + O(\epsilon^3))$$
Now note that the integral we want to evaluate is $$e^{2 \theta m} e^{-2\theta n} \frac{n!}{2 \pi i} \lam_0^{-n} \int_{-\pi}^\pi h(\psi) d\psi$$

where $$h(\psi) = e^{-n i \psi} \prod_{j=1}^m (e^{\lam_0 \nu_j e^{i\psi}} - 1 + e^{-2\theta})$$

so, $H(\psi)$ is same as before. We can show that 

$$Re(H(0)) = n - 2 \theta e^{-n/m} (m+n) + 2 \theta^2 \frac{e^{-2n/m} (-m^2 + e^{n/m} m^2 - 2 m n + e^{n/m} m n - 2n^2)}{m} + O(\eps^3)$$

(Last term is probably actually $O(m\eps^3) = o(m \eps^2)$ - have to check this using Mathematica.
%$$Re(H(0)) = \lam_0 - 2 m\theta e^{-\frac{n}{m}} + O(n \eps^2)$$
$$H''(\psi) = -n e^{i \psi} + O(n \eps)$$


==> eric_scratch.tex <==
\section{Eric's scratch}

  \xxx{ERIC'S SCRATCH: QUESTIONS}

  Is
  \[
    g(S, \theta) := \E[e^{\theta S - \theta \E[S] - \theta^2 \Var[S]/2}] = e^{o(m)}?
  \]
  Questions: can we replace $S_n$ with $S_{poi(n)}$ here?  Because if
  we shift moments, then the $\E[S_{poi(n)}^l]$ is much less nice.

  Suggested lemma, at least for $\theta > 0$:
  \[
    g(S_n, \theta) \leq g(S_{poi(n)}, 2\theta).
  \]


  Both expectations are $n$.  Poissonized variance is $n + 2n^2/m$.  Nonpoissonized is $n^2/2m - n^2/m^2 ~= n^2/(2m)$ for $sum (Yj choose 2)$, but nonpoissonized $\sum Yj^2 = 2n^2/m$.  [Q: why don't variances match when $n \ll m?$]
  For the poissonized statistic:
  \[
    \E[e^{\theta S}] = 1 + \theta \E[S] + \theta^2/2 \Var[S] + o(1) = 1 + theta n + (theta^2/2) \cdot \Theta(n^2/m) + o(n^2/m) = f(\theta, S) + o(n^2/m).
  \]

  % \xxx{NOTE 1.} By AM-GM,
  % \[
  %   \E_S \E_{\pm k}[e^{\theta (S_{n \pm k})}] \geq \E_S [e^{\theta \E_{\pm k}[ S_{n \pm k}]}] \geq \E_S [e^{\theta S_n}]
  % \]
  % where the last step needs $\theta > 0$.

  [Huang-Meyn: 1 if $Y_j = 1$, 0 otherwise.  Poissonized variance is
  $\approx n$, as is depoissonized variance.  But they have
  $\lambda_0 = (1 - \eps^2)n$ and $\eps$ can be constant? I guess the
  claim is that the mean term is better, which decreases the
  variance...]

  \xxx{Note 2.}  Suggestion is:  Define
  \[
    f(\theta, S) := 1 + \theta \E[S] + \theta^2/2 \E[S^2]
  \]
  and
  \[
    g(\theta, S) := \E[e^{\theta S}] - f(\theta, S)
  \]
  and
  \[
    h(\theta, S) := \E[e^{\theta S - (\theta \E[S] + \theta^2/2 \Var[S])}]
  \]


==> failed_attempts.tex <==
\section{Failed attempts}

\subsection{Proving bounds for variables in $W_j$ in terms of $Z_j$}
It's not necessarily the case that $f \le g$ implies $|\E[f(W_j)]| \le |\E[g(W_j)]|$. So, proving \ref{lem:quadratic_terms_bound} seems to not be straightforward. Similar problems with remaining higher moments bounds section

\subsection{Looking at $G(\psi)$ and derivatives}
It seems that the current calculations for derivatives of $G(\psi) = \log(g(\psi))$ (in Lemma \ref{lem:G_second_derivative}) should hold, because they involved ratios of expectations in terms of $W_j$. To see, why, note that $$\left|\frac{\E[f(W_j)]}{\E[g(W_j)]}\right| = \left| \frac{\sum_{k=0}^\infty \frac{\lam e^{i\psi}}{k!} e^{-\lam e^{i \psi}} f(k) }{\sum_{k=0}^\infty \frac{\lam e^{i\psi}}{k!} e^{-\lam e^{i \psi}} g(k) }\right| = \frac{|\sum_{k=0}^\infty \frac{\lam e^{i \psi}}{k!} e^{-\lam} f(k)|}{|\sum_{k=0}^\infty \frac{\lam e^{i \psi}}{k!} e^{-\lam} g(k)|} = \frac{\E[|f(Z_j)|]}{\E[|g(Z_j)|]} $$

However, since $G(\psi)$ itself is not written in terms of a ratio, I don't know how to calculate it for $\psi \neq 0$. From the above, we can try and write $$G(\psi) = G(0) + G'(0) \psi + G''(\Tilde \psi) \psi^2$$
for some $\Tilde \psi \in (0, \psi)$.

It would be sufficient to show that $G(\psi) < G(0)$ for all $\psi \in [\pi/3, \pi] \cup [-\pi, -\pi/3]$. We have from our calculation that $G''(\psi) = -n e^{i \psi}$, and $G'(0) = 0$. So, this doesn't quite work (i.e., the approximation centered at $0$ is not good enough for our whole range), since $G''(\psi) > 0$ for $\psi > \pi/2$.

\textbf{Potential idea:} Maybe evaluating $G(\pi)$ is enough, since we can Taylor expand around $\pi$? But I don't know how to do this.

\subsection{Try and Taylor expand expressions}

I think this doesn't work at all but:

$$e^{-i n \psi} \prod_{j=1}^m \left[ \sum_{k=0}^\infty \frac{(\lam_0 \nu_j e^{i \psi})^k}{k!} e^{\eps^2 \theta S(k)}\right] = e^{-i n \psi} \prod_{j=1}^m \left[ \sum_{k=0}^\infty \frac{(\lam_0 \nu_j e^{i \psi})^k}{k!} (1 + \eps^2 \theta S(k) + \frac{\eps^4 \theta^2}{2} S(k)^2 + stuff)\right]$$

But evaluating this ends up being the same as before, there doesn't seem to be much more you can do here.

==> failed_rewrite.tex <==
\section{Rewrite}

%\begin{lemma}
%\label{lem:poisson_naive_bound}
%For non-negative $f(\cdot)$, we have that $\E[f(S_n)] \le \frac{\E[f(S_{Poi(n)})]}{\Pr[Z = n]}$ where $Z \sim Poi(n)$.
%\end{lemma}
%
%\begin{proof}
%$$\E[f(S_{Poi(n)}] = \sum_{k=0}^\infty \E[f(S_k)] \Pr[Z = k] \ge \E[f(S_n)] \Pr[Z=n]$$
%The claim follows.
%\end{proof}

\begin{lemma}
$$|\E[f(S_{Poi(n e^{i \psi}})]| \le \E[|f(S_{Poi(n)})|]$$
\end{lemma}

\begin{proof}
We have 
\begin{align*}
|\E[f(S_{Poi(n e^{i \psi}})]| &= \left| \sum_{k=0}^\infty \frac{(n e^{i \psi})^k}{k!} e^{-n e^{i \psi}} f(S_k) \right|
\end{align*}
Taylor expanding $e^{-n e^{i \psi}}$, this is
\begin{align*}
&= \left|\sum_{k=0}^\infty \frac{(ne^{i \psi})^k}{k!} \left[ \sum_{l=0}^\infty \frac{(-n e^{i \psi})^l}{l!} \right] f(S_k)\right|\\
&= \left|\sum_{k=0}^\infty \sum_{l=0}^\infty \frac{n^{k} (-n)^l e^{i \psi (k + l)}}{k! l!} f(S_k) \right|\\
&\le \sum_{k=0}^\infty \sum_{l = 0}^\infty
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:little_o_depoissonization}
Suppose we have $f$ such that $\E[f(S_{Poi(n)})] = o\left(\frac{n^2 \eps^4}{m}\right)$. Then, $|\E[f(S_n)]| = o\left(\frac{n^2 \eps^4}{m}\right)$.
\end{lemma}
\begin{proof}
\textbf{Notation:} For $\psi \in \R$, we define $$\E[f(\Tilde S)] = \E[f(S_{Poi(n e^{i \psi})})] := \sum_{k=0}^\infty \frac{(n e^{i \psi})^k e^{-n e^{i\psi}}}{k!} f(S_k)$$

By Cauchy's integral formula, We have that 
\begin{align*}
\E[f(S_n)] &= \frac{n!}{2 \pi i} \oint \frac{e^\lam}{\lam^{n+1}} \E[f(S_{Poi(\lam)})] d\lam\\
%&= \frac{n!}{2 \pi i} \oint \frac{e^\lam}{\lam^{n+1}} o\left(\frac{n^2 \eps^4}{m} \right) d\lam\\
%&= o\left(\frac{n^2 \eps^4}{m} \right)
\end{align*}

Choosing the loop passing through $\lam_0 = n$, so that we let $\lam = n e^{i \psi}$ we have 
\begin{align*}
\E[f(S_n)] &= \frac{n!}{2 \pi} \int_{0}^{2 \pi} \frac{e^{n e^{i \psi}}}{n^n} e^{-n i \psi} \E[f(S_{Poi(n e^{i\psi})})]d \psi\\
%&= \frac{n!}{2 \pi} \int_0^{2 \pi} \frac{e^{n e^{i \psi}}}{n^n} e^{-n i \psi} \left[\sum_{k=0}^\infty \frac{(n e^{i \psi})^k e^{-n e^{i \psi}}}{k!} \E[f(S_k)]\right] d \psi\\
&= \frac{n!}{2 \pi n^n} \int_0^{2 \pi} e^{H(\psi)} d\psi
%&= \frac{n!}{2 \pi} \int_0^{2 \pi} \frac{e^{-n i \psi}}{n^n} \left[\sum_{k = 0}^\infty \frac{(n e^{i \psi})^k}{k!} \E[f(S_k)]\right] d \psi\\
\end{align*}

where $$H(\psi) = - i n \psi + n e^{i \psi} + \log\{\E[f(S_{Poi(n e^{i \psi})}]\}$$

By Lemma \ref{lem:squared_huber_H_derivatives}, we have $$H'(\psi) = - i n + i n e^{i \psi} \frac{\E[f(S_{Poi(n e^{i \psi})} + 1)]}{\E[f(S_{Poi(n e^{i \psi})})]}$$

so that $Re(H'(0)) = 0$, and $$H''(\psi) = \frac{(n e^{i \psi})^2 \left\{ \E[f(\Tilde S + 1)]^2 - \E[f(\Tilde S)] \E[f(\Tilde S + 2)]\right\} - (n e^{i \psi})\E[f(\Tilde S)] \E[f(\Tilde{S} + 1)]}{\E[f(\Tilde S)]^2}$$

Now, $$|\E[f(S_{Poi(n e^{i\psi})})| \le \E[f(S_{Poi(n)})] = o\left(\frac{n^2 \eps^4}{m}\right)$$

Thus, $$|\E[f(S_n)]| = o\left(\frac{n^2 \eps^4}{m} \right) \frac{n!}{2 \pi i} \oint \frac{e^\lam}{\lam^{n+1}} d \lam = o\left(\frac{n^2 \eps^4}{m}\right)$$

%So, we have $$|\E[f(S_n)]| \le \frac{n!}{2 \pi} \int_{0}^{2 \pi} \frac{e^{n e^{i \psi}}}{n^n e^{i n \psi}} d\psi$$
\end{proof}

To compute: $$\E[e^{\theta \Tilde{S}}] = e^{\theta \E[\Tilde{S}] + \frac{\theta^2}{2} \Var[\Tilde{S}] + O(\theta^3 \E[\Tilde{S}^3])}$$ 

Let $Z \sim Poi(n)$ be the number of balls drawn. Now, by law of total variance $$\Var[\Tilde{S}_{Poi(n)}] = \E[\Var[\Tilde S_{Poi(n)} | Z]] + \Var[\E[\Tilde S_{Poi(n)} | Z]]$$

So, $$\E[\Var[\Tilde S_{Poi(n)} | Z]] = \Var[\Tilde S_{Poi(n)}] - \Var[\E[\Tilde{S}_{Poi(n)} | Z]]$$

Here, for collisions/Huber, for the uniform distribution $$\E[S_{Poi(n)} | Z] \approx \binom{Z}{2} \|p\|_2^2 = \frac{Z^2 - Z}{2m}$$



$$\Var[\Tilde{S}_{Poi(n)} | Z] \approx Z^2 \|p\|_2^2 + Z^3 (\|p\|_3^3 - \|p\|_2^4)$$

Computing this, we get $$\E[\Var[\Tilde{S}_{Poi(n)} | Z]] = n - \frac{n^2}{2m}$$

\subsection{Poissonization}

We have that the poissonized MGF is $$\E[e^{\theta \Tilde{S}}] = e^{\theta \E[\Tilde{S}]} + \frac{\theta^2}{2} \Var[\Tilde{S}] + O(\theta^3 \E[\Tilde{S}^3])$$

\subsection{Depoissonization}

$$\E[e^{\theta S}] = $$

\subsection{Another approach}

$$\E[e^{\theta S}] = e^{\theta \E[S]} + \frac{\theta^2}{2} \Var[S] + O(\theta^3 \E[S^3])$$

assuming $\theta^k \E[S^k] \to 0$.

Now, 

Suppose we have $f$ such that $$\E[f(Z_j)] = O(g)$$

\subsection{Supermodularity}
\begin{definition}[NCSS statistic]
\label{def:price_statistic}
We call a statistic $S$ non-negative, convex, symmetric, and separable (NCSS) if we can write $$S(X) = \sum_{j=1}^m f(Y_j)$$
where $Y_j =\sum_{i=1}^n \1_{X_i = j}$, and $f$ is non-negative and convex.
\end{definition}
%\begin{definition}
%For $X$ a configuration of $n-k$ balls to $m$ bins, and $X_1, X_2,$ configurations of $k$ balls to $m$ bins, a function $f$ is supermodular if $$f(X) + f(X \cup X_1 \cup X_2) \ge f(X \cup X_1) + f(X \cup X_2)$$
%\end{definition}
%
%\begin{lemma}
%For a symmetric, convex statistic of the form $$S = \sum_{j=1}^m f(Y_j)$$ where $f$ is convex, we have that $S$ is supermodular
%\end{lemma}
%
%\begin{proof}
%Let $A_j = \sum_{i=1}^n \1_{X_i = j}$, $B_j = \sum_{j=1}^n \1_{X_{1, i} = j}$ and $C_j = \sum_{j=1}^n \1_{X_{2, i} = j}$. 
%By convexity, we have that $$f(x + a) \le \frac{b}{a + b} f(x) + \frac{a}{a + b} f(x + a + b)$$
%and $$f(x + b) \le \frac{a}{a + b} f(x) + \frac{b}{a + b} f(x + a + b)$$
%
%Thus, $$f(x) + f(x + a + b) \ge f(x + a) + f(x + b)$$
%
%So, 
%\begin{align*}
%S(X) + S(X \cup X_1 \cup X_2) &=\sum_{j=1}^m \left\{f(A_j) + f(A_j + B_j + C_j)\right\} \\
%&\ge \sum_{j=1}^m \left \{ f(A_j + B_j) + f(A_j + C_j)\right\} = S(X \cup X_1) + S(X \cup X_2)\\
%\end{align*}
%\end{proof}

\begin{lemma}
\label{lem:convex_bound}
For a convex function $f$, and $x, a, b \ge 0$, we have that $$f(x) + f(x + a + b) \ge f(x + a) + f(x + b)$$
\end{lemma}

\begin{proof}
By convexity,
$$f(x + a) \le \frac{b}{a + b} f(x) + \frac{a}{a + b} f(x + a + b)$$.
Similarly, $$f(x + b) \le \frac{a}{a + b} f(x) + \frac{b}{a + b} f(x + a + b)$$.
The claim follows.
\end{proof}
\begin{lemma}
\label{lem:generalized_supermodularity}
For an NCSS statistic $S$, we have $$2^l \left\{S^l(X) + S^l(X \cup X_1 \cup X_2)\right\} \ge S^l(X \cup X_1) + S^l (X \cup X_2)$$
\end{lemma}
\begin{proof}
 Let $A_j = \sum_{i=1}^n \1_{X_i = j}$, $B_j = \sum_{i=1}^n \1_{X_{1, i} = j}$ and $C_j = \sum_{i=1}^n \1_{X_{2, i} = j}$. We have
 $$S(X) + S(X \cup X_1 \cup X_2) = \sum_{j=1}^m \left\{f(A_j) + f(A_j + B_j + C_j) \right\}$$
 By Lemma \ref{lem:convex_bound}, this is at least $$\sum_{j=1}^m \left\{f(A_j + B_j) + f(A_j + C_j)\right\} = S(X \cup X_1) + S(X \cup X_2)$$
 So, we have 
 \begin{align*}
 S^l(X) + S^l(X\cup X_1 \cup X_2) \ge \max\left\{S(X), S(X \cup X_1 \cup X_2) \right\}^l\\
 \ge \left(\frac{S(X) + S(X \cup X_1 \cup X_2)}{2}\right)^l \ge \left(\frac{S(X\cup X_1) + S(X \cup X_2)}{2}\right)^l
 \end{align*}
 By non-negativity of $S$, this is at least $$\frac{S^l(X \cup X_1) + S^l(X \cup X_2)}{2^l}$$.
\end{proof}
%\begin{lemma}
%For a convex (in $Y_j$s) function $S$, we have that $S$ is supermodular
%\end{lemma}
%
%\begin{proof}
%$$S(A_1 + B_1, \dots, A_m + B_m) \le S(A_1$$
%\end{proof}

\begin{lemma}
  For an NCSS statistic $S$, we have that $$2^l \left\{\E[S_{n+k}^l] + \E[S_{n-k}^l]\right\} \ge 2\E[S_n^l]$$.
  \xxx{$S(X)$ isn't $S_n$; need to define $S_n$.}
\end{lemma}

\begin{proof}
By Lemma \ref{lem:generalized_supermodularity}, we have that for any $X$, $X_1, X_2$ such that $|X| = n-k$ and $|X_1| = |X_2| = k$, $$2^l\left\{S^l(X) + S^l(X \cup X_1 \cup X_2)\right\} \ge S^l(X \cup X_1) + S^l(X \cup X_2)$$
Taking expectation over $X, X_1, X_2$, we have the claim.
\end{proof}

\begin{lemma}
\label{lem:Depoissonization_bound}
For a NCSS statistic $S$, as defined in Definition \ref{def:price_statistic}, we have
$$\E[S_n^l] \lesssim 2^{l}\E[S_{Poi(n)}^l]$$
for $n$ larger than a universal constant.\xxx{Not convinced you actually need $n$ above a universal constant.}
\end{lemma} 

\begin{proof}
First, we have that for $Z \sim Poi(n)$ 
\begin{align*}
Pr[Z = n+k] &= \frac{e^{-n} n^{n+k}}{(n+k)!}\\
\end{align*}
For $n$ large enough and $-2 \sqrt{n} \le k \le 2 \sqrt{n}$, by Stirling's approximation, this is at least
\begin{align*}
&\frac{e^{-n} n^{n+k}e^{n+k}}{ (n+k)^{n+k} 2 \sqrt{ \pi (n+k)}}\\
&= \frac{e^k}{\left( 1 + \frac{k}{n} \right)^{n+k} 2 \sqrt{\pi(n+k)}} \ge \frac{e^{-\frac{k^2}{n}}}{2 \sqrt{\pi (n+k)}} \gtrsim \frac{e^{-\frac{k^2}{n}}}{\sqrt{n}}\\
\end{align*}
%For $k \le 2 \sqrt{n}$, this is $$e^{-\frac{k^2}{n}}\sqrt{\frac{2}{\pi n}}$$
So, we have, using the non-negativity of $S$,
\begin{align*}
2^{l} \E[S_{Poi(n)}^l] &\ge 2^{l} \sum_{k = - 2\sqrt{n}}^{2 \sqrt{n}} \Pr[Z = n + k] \E[S_{n+k}^l]\\
&\ge 2^{l} \sum_{k=1}^{2\sqrt{n}} \left\{\Pr[Z = n - k] \E[S_{n-k}^l] + \Pr[Z = n+k] \E[S_{n+k}^l] \right\}\\
&\gtrsim 2^{l} \sum_{k=1}^{2 \sqrt{n}} \left\{ \frac{e^{-\frac{k^2}{n}}}{ \sqrt{n}} \left[\E[S_{n-k}^l] + \E[S_{n+k}^l] \right]\right\}\\
\end{align*}

By Lemma \ref{lem:generalized_supermodularity}, we have
\begin{align*}
   2^{l} \E[S_{Poi(n)}] &\gtrsim \sum_{k=1}^{2 \sqrt{n}} \left\{\frac{e^{-\frac{k^2}{n}}}{\sqrt{n}} \left[ 2 \E[S_n^l]\right] \right\}\\
   &\gtrsim \E[S_n^l] \sum_{k=1}^{2 \sqrt{n}} \frac{e^{-4}}{\sqrt{n}} \\
   &\gtrsim \E[S_n^l]
\end{align*}
\end{proof}
\begin{lemma}
For a non-negative statistic $S$, we have 
$$L(\theta) \le \E[e^{\theta S}] \le U(\theta)$$
where $$L(\theta) := e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 - \sum_{l = 2}^\infty \frac{\theta^{2l}\E[S^{2l}]}{l!}\right)$$
and $$U(\theta) := e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 + \sum_{l = 3}^\infty \frac{\theta^l\E[S^l]}{l!}\right)$$
\xxx{Is the distinction between these error terms important?  If not, it's confusing.}
\xxx{Is there a problem when $\theta < 0$?}
%$$e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 - \sum_{l = 2}^\infty \frac{\theta^{2l}\E[S^{2l}]}{l!}\right) \le \E[e^{\theta S}] \le e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 + \sum_{l = 3}^\infty \frac{\theta^l\E[S^l]}{l!}\right)$$
\end{lemma}
\begin{proof}
%For simplicity, let $$L(\theta) := e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 - \sum_{l = 2}^\infty \frac{\theta^{2l}\E[S^{2l}]}{l!}\right)$$
%and $$U(\theta) := e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 + \sum_{l = 3}^\infty \frac{\theta^l\E[S^l]}{l!}\right)$$
\textbf{Notation:} For a power series $f(x)$, we use $[x^k] f(x)$ to denote the coefficient of $x^k$ in $f(x)$.
We have that $$[1] \E[e^{\theta S}] = 1 = [1] U(\theta) = [1]L(\theta)$$
$$[\theta] \E[e^{\theta S}] = \theta \E[S] = [\theta] U(\theta) = [\theta] L(\theta)$$
$$[\theta^2] \E[e^{\theta S}] = \frac{\E[S^2]}{2} = \frac{\Var[S] + \E[S]^2}{2} = [\theta^2] U(\theta) = [\theta^2] L(\theta)$$
For $l \ge 3$, by non-negativity of $S$, $$[\theta^l] \E[e^{\theta S}] = \frac{\E[S^l]}{l!} \le [\theta^l] U(\theta)$$

Thus, we have the upper bound on $\E[e^{\theta S}]$. For the lower bound, \xxx{I'm having trouble following this argument and the next-- perhaps expand $[\theta^l] L(\theta)$?} for odd $l \ge 3$, by Jensen's inequality and the non-negativity of $S$,
$$[\theta^l]\E[e^{\theta S}] = \frac{\E[S^l]}{l!} \ge \frac{E[S]^l}{l!} \ge [\theta^l]L(\theta)$$
On the other hand, for even $l \ge 3$, by non-negativity of $S$, $$[\theta^l]\E[e^{\theta S}] = \frac{\E[S^l]}{l!} \ge \frac{\E[S]^l}{l!} + \frac{\Var[S]^{l/2}}{2^{l/2} (l/2)!} - \frac{\E[S^{l}]}{(l/2)!} \ge [\theta^l] L(\theta)$$
since by convexity, $\E[S^l] \ge \E[S]^l$, and also by convexity and non-negativity of $S$, $$\frac{\E[S^l]}{(l/2)!} \ge \frac{\E[S^l]}{2^{l/2} (l/2)!} \ge \frac{\E[S^2]^{l/2}}{2^{l/2} (l/2)!} \ge \frac{\Var[S]^{l/2}}{2^{l/2}(l/2)!}$$

So, finally, we have the lower bound on $\E[e^{\theta S}]$.


\xxx{XXX eric working out the even terms.}
\begin{align*}
  [\theta^{2l}] e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]}
  &= \sum_{j=0}^{l} [\theta^{2l}] \frac{1}{(j+l)!} (\theta \E[S] + \frac{\theta^2}{2} \Var[S])^{j+l}\\
  &= \sum_{j=0}^{l} \frac{1}{(j+l)!} \binom{j+l}{2j} \E[S]^{2j}\left(\frac{\Var[S]}{2}\right)^{l-j}
\end{align*}
On the other hand,
\[
  \E[S^2]^l = (\E[S]^2 + \Var[S])^l = \sum_{j=0}^l \binom{l}{j} \E[S]^{2j} \Var[S]^{l-j}.
\]
Comparing these termwise, since
\[
  \frac{1}{(j+l)!} \binom{j+l}{2j} \frac{1}{2^{l-j}} = \frac{1}{(2j)! 2^{l-j} (l-j)!} = \binom{l}{j} \cdot \frac{j!}{l! (2j)! 2^{l-j}} \leq \frac{1}{l! 2^l} \binom{l}{j}
\]
we have
\[
  \frac{1}{l! 2^l} \E[S^2]^l \geq [\theta^{2l}] e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]}.
\]
Thus, for $l \geq 2$,
\[
  [\theta^{2l}] L(\theta) \leq \left([\theta^{2l}] e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]}\right) - \frac{\E[S^{2l}]}{l!} \leq 0.
\]
\end{proof}

\begin{proof}
  \xxx{ERIC'S SCRATCH: QUESTIONS}

  Is
  \[
    g(S, \theta) := \E[e^{\theta S - \theta \E[S] - \theta^2 \Var[S]/2}] = e^{o(m)}?
  \]
  Questions: can we replace $S_n$ with $S_{poi(n)}$ here?  Because if
  we shift moments, then the $\E[S_{poi(n)}^l]$ is much less nice.

  Suggested lemma, at least for $\theta > 0$:
  \[
    g(S_n, \theta) \leq g(S_{poi(n)}, 2\theta).
  \]


  Both expectations are $n$.  Poissonized variance is $n + 2n^2/m$.  Nonpoissonized is $n^2/2m - n^2/m^2 ~= n^2/(2m)$ for $sum (Yj choose 2)$, but nonpoissonized $\sum Yj^2 = 2n^2/m$.  [Q: why don't variances match when $n \ll m?$]
  For the poissonized statistic:
  \[
    \E[e^{\theta S}] = 1 + \theta \E[S] + \theta^2/2 \Var[S] + o(1) = 1 + theta n + (theta^2/2) \cdot \Theta(n^2/m) + o(n^2/m) = f(\theta, S) + o(n^2/m).
  \]

  % \xxx{NOTE 1.} By AM-GM,
  % \[
  %   \E_S \E_{\pm k}[e^{\theta (S_{n \pm k})}] \geq \E_S [e^{\theta \E_{\pm k}[ S_{n \pm k}]}] \geq \E_S [e^{\theta S_n}]
  % \]
  % where the last step needs $\theta > 0$.


  \xxx{Note 2.}  Suggestion is:  Define
  \[
    f(\theta, S) := 1 + \theta \E[S] + \theta^2/2 \E[S^2]
  \]
  and
  \[
    g(\theta, S) := \E[e^{\theta S}] - f(\theta, S)
  \]
  and
  \[
    h(\theta, S) := \E[e^{\theta S - (\theta \E[S] + \theta^2/2 \Var[S])}]
  \]

  Our final goal here is to show that
  \[
    h(\theta, S_n) = e^{o(a)}.
  \]
  where
  \[
    a := \theta \E[S] + \theta^2/2 \Var[S].
  \]
  ( Not sure what other assumptions we need.)

  But, as observed below, $g$ is not small.

  So, we can analyze the Poisson MGF relatively easily, which hopefully shows that
  \[
    h(\theta, S_{Poi(n)}) = e^{o(a)}.
  \]

  We have that
  \[
    [\theta^{2l}]h(\theta, S) \approx \frac{1}{(2l)!}\E[S^{2l}] + \frac{1}{l!} \left( - \E[S^2]^l + \sum_j (1-\frac{2^j j!}{(2j)!}) \cdot C_j\right) \geq XXX
  \]
  for any statistic.  The problem is that $2l!$ is much bigger than $l!$.
  %Assuming the same holds for odd $l$, we only
%  need to upper bound $h$ over positive $\theta$.


  Perhaps we should use $S' = S - \E[S]$.  Then
  \[
    h(\theta, S) = h(\theta, S') = \E[e^{\theta S' - \frac{\theta^2}{2} \E[(S')^2]}]
  \]
  which is rather simpler since moments have no mean term.  In particular we have directly
  \begin{align*}
    [\theta^{2l}] h(\theta, S) &= \sum_{j=0}^l \frac{(-1)^j}{(2l-j)!}\binom{2l-j}{j}\frac{1}{2^j}\E[(S')^2]^j \E[(S')^{2l-2j}]\\
                               & = \sum_{j=0}^l \frac{(-1)^j}{(2l-2j)!j!2^j}\E[(S')^2]^j \E[(S')^{2l-2j}]\\
                               &\lesssim \frac{1}{l! 2^l} \E[(S')^{2l}]
  \end{align*}
  or, ignoring odd terms,
  \[
    h(\theta, S) \lesssim \E[e^{(S')^2/2}].
  \]
  but this isn't great: $(S')^2$ could very well not have an MGF at
  all due to the square.  We actually want to say that
  $h(\theta, S) = e^{o(\theta^2 \sigma^2)},$ or that
  \[
    \sum_{j=0}^l \frac{(-1)^j}{(2l-2j)!j!2^j}\E[(S')^2]^j \E[(S')^{2l-2j}] \overbrace{\ll}^{??}  \frac{1}{l!}\E[(S')^2]^l.
  \]
  Note that, for $l = 1$, the LHS is zero but each individual term is
  comparable to the RHS.  So the cancellation is important.



  Of course, if we always did get the $l!$ not
  the $(2l)!$, we would have
  $[\theta^{2l}]h(\theta, S) = \frac{1}{l!2^l} \sigma^{2l}$, so $h(\theta, S) =
  e^{\theta^2\sigma^2/2} - \theta^2\sigma^2/2$, which is $1 + o(1)$.
  We also have
  \[
    [\theta^{2l}]h(\theta, S) \leq 
  \]

  Analog of 9.7 for possibly negative S?  Can we say that the poisson
  central moments are bigger than the non-poisson central moments?

  Maybe start with $m = 2$?  So $X \sim B(n, .5)$ and symmetry means
  $S_n = 2\phi(X - n/2)$ while
  $S_{poi} = \phi(X_1 - n/2) + \phi(X_2 - n/2)$ for
  $X_1, X_2 \sim \Poi(n/2)$.  We want to bound $\E[(S - \E[S])^l]$.

  We have
  \[
    \Var[S_{poi(n)}] = \E_{n'}[\Var[S_{n'} \mid n']] + \Var_{n'}[\E[S_{n'} \mid n']]
  \]
  

  THE BELOW IS ALL WRONG.
  To do this, we observe that:
  \begin{enumerate}
  \item $\E[e^{\theta S_{poi(n)}}]$ is easy to compute
  \item This computation gives that $g(\theta, S_{poi(n)})$ is small.
  \item We already have that $\E[S_n^l] \lesssim 2^l \E[S^l_{poi(n)}]$.
  \item For every $\theta$,
    \[
      g(\theta, S_{n})  \leq g(\abs{\theta}, S_{n}) \leq g(2\abs{\theta}, S_{poi(n)}).
    \]
  \end{enumerate}
  As a result,
  \[
    g(\theta, S_n) = o(1).
  \]
  The question becomes: how does this make $h(\theta, S_n) = 1 + o(1)$?  Because
  \[
    e^{\theta \E[S] + \theta^2/2 \Var[S]} = f(\theta, S) + O(\theta^3 \cdot stuff)
  \]
  and we need to say that that last term is $o(1)$.  And it is $o(1)$,
  since $e^a = 1 + a + o(1)$ if $a = o(1)$, as long as
  \[
    \theta \E[S] + \theta^2/2 \Var[S] = o(1).
  \]
  Which really ought to be true, since $\theta \E[S] \approx \eps$.


  Lemma would be:  Suppose that $a := \theta \E[S] + \theta^2/2 \Var[S] \leq 1$ AND $b := g(2\abs{\theta}, S_{Poi(n)}) \leq 1$.  Then
  \[
    \E[e^{\theta S}] = e^{a + O(a^2 + b)}.
  \]

  Doing the MGF for a tail bound gives:
  \[
    Pr[S>\mu + \sigma t] < E[e^{\theta S}]/e^{\theta (\mu + \sigma t)} \approx e^{\theta \mu + \theta^2 \sigma^2/2}/e^{\theta \mu + \theta \sigma t} = e^{(1/2) (\theta^2 \sigma^2 - 2\theta \sigma t)} = e^{(1/2) (\theta \sigma - t)^2 - t^2/2} = e^{-t^2/2}
  \]
  by setting
  $\theta = t/\sigma \approx \sqrt{\log \frac{1}{\delta}} \cdot
  \frac{\sqrt{m}}{n} \approx \eps^2$.  But this means
  $\theta \E[S] = \theta n \approx \sqrt{m \log \frac{1}{\delta}} \gg
  1$, so in fact $e^{\theta S}$ is not well approximated $1 + \theta S + \theta^2 \Var[S]/2$.
  
\end{proof}

\begin{proof}
\begin{align*}
h(\theta, S_{Poi(n)}) &=\prod_{j=1}^m \E[ e^{\theta f(Z_j) - (\theta \E[f(Z_j)] + \frac{\theta^2}{2} \Var[Z_j]) }]\\
&\le \prod_{j=1}^m \left(1 - \theta \E[f(Z_j)] - \frac{\theta^2}{2} \Var[Z_j]\right) \E[e^{\theta f(Z_j)}]\\
& = \prod_{j=1}^m \left( 1 - \theta \E[f(Z_j)] - \frac{\theta^2}{2} \Var[Z_j]\right) \sum_{l=0}^\infty \frac{\theta^l \E[f(Z_j)^l]}{l!}\\
&= \prod_{j=1}^m \left(1 + \sum_{l=3}^\infty \frac{\theta^l \E[f(Z_j)^l]}{l!} \right)
\end{align*}

\end{proof}

\begin{corollary}
For a NCSS statistic $S$, we have $$L(\theta) \le \E[e^{\theta S}] \le U(\theta)$$
where $$L(\theta) := e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 - O\left(\sum_{l = 2}^\infty \frac{(2\theta)^{2l}\E[S_{Poi(n)}^{2l}]}{l!}\right)\right)$$
and $$U(\theta) := e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 + O\left(\sum_{l = 3}^\infty \frac{(2\theta)^l\E[S_{Poi(n)}^l]}{l!}\right)\right)$$
\end{corollary}
\begin{proof}
Follows from Lemma \ref{lem:Depoissonization_bound}.
\end{proof}
%\begin{lemma}
%For a NCSS statistic $S$, as defined in Definition \ref{def:price_statistic}, such that $\theta \E[S] = O\left(\frac{n\eps^2}{m}\right)$, $\theta^2 \Var[S] = O(\frac{n^2\eps^4}{m})$ and $\sum_{l=3}^\infty \frac{\theta^l}{l!} \E[S_{Poi(n)}^l] = o\left(\frac{n^2 \eps^4}{m}\right)$, we have that 
%%$$\E[e^{\theta S}] = \exp\left\{\theta \E[S] + \frac{\theta^2}{2} \Var[S] + o\left(\frac{n^2 \eps^4}{m} \right)\right\}$$
%$$e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 - \sum_{l = 2}^\infty \frac{\theta^{2l}\E[S^{2l}]}{l!}\right) \le \E[e^{\theta S}] \le e^{\theta \E[S] + \frac{\theta^2}{2} \Var[S]} \left(1 + \sum_{l = 3}^\infty \frac{\theta^l\E[S^l]}{l!}\right)$$
%\end{lemma}
%
%\begin{proof}
%By Taylor expansion,
%$$\E[e^{\theta S}] = 1 + \theta \E[S] + \frac{\theta^2}{2} \E[S^2] + \sum_{l=3}^\infty \frac{\theta^l}{l!} \E[S^l]$$
%
%Now, by Lemma \ref{lem:little_o_depoissonization}, since $\sum_{l=3}^\infty \frac{\theta^l}{l!}\E[S_{Poi(n)}^l] = o\left(\frac{n^2 \eps^4}{m}\right)$, we have that $$\sum_{l=3}^\infty \frac{\theta^l}{l!} \E[S^l] = o\left(\frac{n^2 \eps^4}{m} \right)$$
%
%Now, $$\E[e^{\theta S}] = 1 + \theta \E[S] + \frac{\theta^2}{2} \E[S^2] + o\left(\frac{n^2 \eps^4}{m} \right)$$
%$$ = \exp\left\{\theta \E[S] + \frac{\theta^2}{2} \Var[S] + o\left(\frac{n^2 \eps^4}{m} \right)\right\}$$
%
%\end{proof}
\subsection{Expectation and Variance computation}
\subsubsection{Collisions Statistic}
\begin{lemma}[From \cite{DGPP19}]
\label{lem:collisions_expectation_variance}
For the collisions statistic $S = \sum_{j=1}^m \binom{Y_j}{2}$, we have $$\E_p[S] = \binom{n}{2} \|p\|_2^2$$
$$\Var_p[S] = \binom{n}{2} \left( \|p\|_2^2 - \|p\|_2^4\right) + n(n-1)(n-2) \left(\|p\|_3^3 - \|p\|_2^4 \right)$$
\end{lemma}

\subsubsection{Huber Statistic}
\begin{lemma}[Bernstein's inequality]
\label{lem:bernstein_inequality}
For random variable $X$ with $\sigma^2 = \Var(X)$ and $\mu = \E[X]$, such that $|X - \mu| \le m$ we have that $$\Pr[|X - \mu| \ge t] \le 2 \max\left(e^{-\frac{t^2}{4 \sigma^2}}, e^{\frac{-t}{4m}} \right)$$
\end{lemma}
\begin{lemma}
\label{lem:huber_expectation_variance_lower_bound}
For statistic $S = \sum_{j=1}^m \1_{\{\phi(Y_j) \le \beta\}} \binom{Y_j}{2}$, with $\beta$ satisfying \eqref{eq:beta_second_bound} and \eqref{eq:beta_third_bound}, and $p$ such that $p_j = 1/m + O(\eps/m)$ for all $j$, we have
$$\E_p[S] = (1 + o(1)) \binom{n}{2} \|p\|_2^2$$
$$\Var_p[S] = (1 + o(1)) \left\{\binom{n}{2} \left( \|p\|_2^2 - \|p\|_2^4\right) + n(n-1)(n-2) \left(\|p\|_3^3 - \|p\|_2^4 \right) \right\}$$
\end{lemma}
\begin{proof}
We can write this statistic as 
\begin{equation}
\label{eq:collisions_statistic_alternate_form}
S = \sum_{i, j} \1_{\{\phi(Y_{X_i}) \le \beta\}} \sigma_{ij}
\end{equation}
where $\sigma_{ij} = \1_{\{X_i = X_j\}}$.

Then, $$\E_p[S] = \sum_{i, j} \E_p[\1_{\left\{\phi(Y_{X_i}) \le \beta\right\}} \sigma_{ij}] = \sum_{i, j} \E_p[\sigma_{ij}] \E[\1_{\{\phi(Y_{X_i}) \le \beta\}} | \sigma_{ij} = 1]$$

Now, $$\E_p[\1_{\{\phi(Y_{X_i}) \le \beta\}} | \sigma_{ij} = 1] = \Pr_p\left[\phi(Y_{X_i}) \le \beta | \sigma_{ij} = 1\right]$$

This is the probability that bin $X_i$ receives at least $\frac{n}{m} - \beta-2$ and at most $\frac{n}{m} + \beta-2$ balls if $n-2$ balls are thrown. Since $p_{X_i} = 1/m + O(\eps/m)$, and $\beta$ satisfies \eqref{eq:beta_second_bound} and \eqref{eq:beta_third_bound}, by Bernstein's inequality (Lemma \ref{lem:bernstein_inequality}), this happens with probability at least $1 - O(\Delta^{2 \eta}) = 1 + o(1)$ for constant $\eta$. Thus, $$\E_p[S] = (1 + o(1)) \sum_{i, j} \E_p[\sigma_{ij}] = (1 + o(1)) \E_p\left[\sum_{j=1}^m \binom{Y_j}{2}\right]$$
By Lemma \ref{lem:collisions_expectation_variance}, the claim for the expectation follows.

For the variance, we begin by computing $\E_p[S^2]$ using \eqref{eq:collisions_statistic_alternate_form}. \begin{align*}
    \E_p[S^2] &= \E_p\left[\left(\sum_{i, j}\1_{\{\phi(Y_{X_i}) \le \beta\}} \sigma_{ij}\right)^2\right]\\
    &= \sum_{i < j} \sum_{k < l}\E_p\left[ \1_{\{\phi(Y_{X_i}) \le \beta\}} \1_{\{\phi(Y_{X_k}) \le \beta\}} \sigma_{ij} \sigma_{kl}\right]\\
    &= \sum_{i < j}\sum_{k < l} \E_p[\sigma_{ij} \sigma_{kl}] \E_p[\1_{\{\phi(Y_{X_i}) \le \beta\}} \1_{\{\phi(Y_{X_k}) \le \beta\}} | \sigma_{ij} \sigma_{kl} = 1]
\end{align*}
Now, 
\begin{align*}
\E_p[\1_{\{\phi(Y_{X_i}) \le \beta\}}\1_{\{\phi(Y_{X_k}) \le \beta\}} | \sigma_{ij} \sigma_{kl} = 1] = \Pr_p[\{\phi(Y_{X_i}) \le \beta\}\cap \{\phi(Y_{X_k}) \le \beta\} | \sigma_{ij} \sigma_{kl} = 1]\\
= \Pr_p[\phi(Y_{X_i}) \le \beta | \sigma_{ij} \sigma_{kl} = 1] \Pr_p[\phi(Y_{X_k} \le \beta | \sigma_{ij} \sigma_{kl} = 1, \phi(Y_{X_i}) \le \beta]
\end{align*}
Here, both these terms are at least $1 - O(\Delta^{2 \eta}) = 1 + o(1)$ using Bernstein's inequality, as in the case of the expectation.
So, we have $$\E_p[S^2] = (1 + o(1))\sum_{i < j} \sum_{k < l} \E_p[\sigma_{ij} \sigma_{kl}] = (1 + o(1)) \E_p\left[\left(\sum_{j=1}^m \binom{Y_j}{2} \right)^2 \right]$$

Now, using the expectation bound, $$\E[S]^2 = (1 + o(1)) \E_p\left[ \sum_{j=1}^m \binom{Y_j}{2} \right]^2$$

So, $$\Var_p[S] = (1 + o(1)) \Var_p\left[\sum_{j=1}^m\binom{Y_j}{2}\right]$$
By Lemma \ref{lem:collisions_expectation_variance}, the bound follows.
\end{proof}
\begin{lemma}
For the Huber statistic $S = \sum_{j=1}^m h_\beta\left(Y_j - \frac{n}{m}\right)$, with $\beta$ satisfying \eqref{eq:beta_second_bound} and \eqref{eq:beta_third_bound}, and $p$ such that $p_j = 1/m + O(\eps/m)$ for all $j$, we have
$$\E_p[S] =(1 + o(1)) \left\{ 2\binom{n}{2} \|p\|_2^2 + n - \frac{n^2}{m}\right\}$$
$$\Var_p[S] = (1 + o(1)) \left\{ \right\}$$
\end{lemma}

\begin{proof}
First, $$\left(Y_j - \frac{n}{m}\right)^2 = 2\binom{Y_j}{2} + Y_j\left(1 - \frac{2n}{m} \right) + \frac{n^2}{m^2}$$
We have
$$S \ge \sum_{j=1}^m \1_{\phi(Y_j) \le \beta} \left(Y_j - \frac{n}{m} \right)^2$$
So, by Lemma \ref{lem:huber_expectation_variance_lower_bound}, we have the lower bound on the expectation and variance.
We also have $$S \le \sum_{j=1}^m \left(Y_j - \frac{n}{m}\right)^2$$
Then, Lemma \ref{lem:collisions_expectation_variance} gives us the matching upper bound (up to o(1)).
\end{proof}

==> notation.tex <==
\section{Notation}

